Model Uncertainty and Correctability for Directed Graphical Models

Probabilistic graphical models are a fundamental tool in probabilistic modeling, machine learning and artificial intelligence. They allow us to integrate in a natural way expert knowledge, physical modeling, heterogeneous and correlated data and quantities of interest. For exactly this reason, multiple sources of model uncertainty are inherent within the modular structure of the graphical model. In this paper we develop information-theoretic, robust uncertainty quantification methods and non-parametric stress tests for directed graphical models to assess the effect and the propagation through the graph of multi-sourced model uncertainties to quantities of interest. These methods allow us to rank the different sources of uncertainty and correct the graphical model by targeting its most impactful components with respect to the quantities of interest. Thus, from a machine learning perspective, we provide a mathematically rigorous approach to correctability that guarantees a systematic selection for improvement of components of a graphical model while controlling potential new errors created in the process in other parts of the model. We demonstrate our methods in two physico-chemical examples, namely quantum scale-informed chemical kinetics and materials screening to improve the efficiency of fuel cells.

==> SIAM_BN_BFKR.bbl_. <==
\begin{thebibliography}{10}

\bibitem{8466590}
Amina Adadi and Mohammed Berrada.
\newblock Peeking inside the black-box: A survey on explainable artificial
  intelligence (xai).
\newblock {\em IEEE Access}, 6:52138--52160, 2018.

\bibitem{antoine2001}
Olivier Antoine, Yann Bultel, and Robert Durand.
\newblock Oxygen reduction reaction kinetics and mechanism on platinum
  nanoparticles inside nafion$^{\textregistered}$.
\newblock {\em Journal of Electroanalytical Chemistry}, 499(1):85--94, 2001.

\bibitem{aronsky1998diagnosing}
Dominik Aronsky and Peter~J Haug.
\newblock Diagnosing community-acquired pneumonia with a bayesian network.
\newblock In {\em Proceedings of the AMIA Symposium}, page 632. American
  Medical Informatics Association, 1998.

\bibitem{pmlr-v80-belghazi18a}
Mohamed~Ishmael Belghazi, Aristide Baratin, Sai Rajeshwar, Sherjil Ozair,
  Yoshua Bengio, Aaron Courville, and Devon Hjelm.
\newblock Mutual information neural estimation.
\newblock In Jennifer Dy and Andreas Krause, editors, {\em Proceedings of the
  35th International Conference on Machine Learning}, volume~80 of {\em
  Proceedings of Machine Learning Research}, pages 531--540. PMLR, 10--15 Jul
  2018.

\bibitem{birmpa2020uncertainty}
Panagiota Birmpa and Markos~A. Katsoulakis.
\newblock Uncertainty quantification for markov random fields.
\newblock {\em arXiv preprint, arXiv: 2009.00038}, 2020.

\bibitem{BDKPRB}
Jeremiah {Birrell}, Paul {Dupuis}, Markos~A. {Katsoulakis}, Yannis {Pantazis},
  and Luc {Rey-Bellet}.
\newblock {$(f,\Gamma)$-Divergences: Interpolating between $f$-Divergences and
  Integral Probability Metrics}.
\newblock {\em arXiv e-prints}, page arXiv:2011.05953, November 2020.

\bibitem{birrell2021variational}
Jeremiah Birrell, Paul Dupuis, Markos~A. Katsoulakis, Luc Rey-Bellet, and Jie
  Wang.
\newblock Variational representations and neural network estimation of r\'enyi
  divergences.
\newblock {\em arXiv preprint, arXiv:2007.03814}, 2021.

\bibitem{Birrell_GOKL}
Jeremiah {Birrell}, Markos {Katsoulakis}, and Luc {Rey-Bellet}.
\newblock {Robustness of Dynamical Quantities of Interest via Goal-Oriented
  Information Theory}.
\newblock {\em arXiv e-prints}, page arXiv:1906.09282, Jun 2019.

\bibitem{Birell-RB2020}
Jeremiah Birrell and Luc Rey-Bellet.
\newblock Uncertainty quantification for markov processes via variational
  principles and functional inequalities.
\newblock {\em SIAM/ASA Journal on Uncertainty Quantification}, 8(2):539--572,
  2020.

\bibitem{bishop}
Christopher~M. Bishop.
\newblock {\em Pattern Recognition and Machine Learning (Information Science
  and Statistics)}.
\newblock Springer-Verlag New York, Inc., Secaucus, NJ, USA, 2006.

\bibitem{BlaLamTangYuan2019}
Jose Blanchet, Henry Lam, Qihe Tang, and Zhongyi Yuan.
\newblock Robust actuarial risk analysis.
\newblock {\em North American Actuarial Journal}, 23(1):33--63, 2019.

\bibitem{doi:10.1287/moor.2018.0936}
Jose Blanchet and Karthyek Murthy.
\newblock Quantifying distributional model risk via optimal transport.
\newblock {\em Mathematics of Operations Research}, 44(2):565--600, 2019.

\bibitem{Burges2016ABC}
C.~Burges, Ted Hart, Zi~Yang, Silviu Cucerzan, Ryen~W. White, A.~Pastusiak, and
  J.~Lewis.
\newblock A base camp for scaling ai.
\newblock {\em arXiv: 1612.07896}, 2016.

\bibitem{callevallejo2015}
Federico Calle-Vallejo, Jakub Tymoczko, Viktor Colic, Quang~Huy Vu, Marcus~D
  Pohl, Karina Morgenstern, David Loffreda, Philippe Sautet, Wolfgang
  Schuhmann, and Aliaksandr~S Bandarenka.
\newblock Finding optimal surface sites on heterogeneous catalysts by counting
  nearest neighbors.
\newblock {\em Science}, 350(6257):185--189, 2015.

\bibitem{dupuis2011uq}
Kamaljit Chowdhary and Paul Dupuis.
\newblock Distinguishing and integrating aleatoric and epistemic variation in
  uncertainty quantification.
\newblock {\em ESAIM: Mathematical Modelling and Numerical Analysis},
  47(03):635--662, 2013.

\bibitem{cover2012elements}
Thomas~M Cover and Joy~A Thomas.
\newblock {\em Elements of information theory}.
\newblock John Wiley \& Sons, 2012.

\bibitem{doi:10.1287/opre.1090.0741}
Erick Delage and Yinyu Ye.
\newblock Distributionally robust optimization under moment uncertainty with
  application to data-driven problems.
\newblock {\em Operations Research}, 58(3):595--612, 2010.

\bibitem{Daskalakis:PGM:2021GANsWC}
Mucong Ding, C.~Daskalakis, and S.~Feizi.
\newblock Gans with conditional independence graphs: On subadditivity of
  probability divergences.
\newblock In {\em AISTATS}, 2021.

\bibitem{DoshiVelez2017TowardsAR}
Finale Doshi-Velez and Been Kim.
\newblock Towards a rigorous science of interpretable machine learning.
\newblock {\em arXiv: 1702.08608}, 2017.

\bibitem{dupuis2011weak}
Paul Dupuis and Richard~S Ellis.
\newblock {\em A weak convergence approach to the theory of large deviations},
  volume 902.
\newblock John Wiley \& Sons, 2011.

\bibitem{dupuis2016path}
Paul Dupuis, Markos~A Katsoulakis, Yannis Pantazis, and Petr Plech{\'a}c.
\newblock Path-space information bounds for uncertainty quantification and
  sensitivity analysis of stochastic dynamics.
\newblock {\em SIAM/ASA Journal on Uncertainty Quantification}, 4(1):80--111,
  2016.

\bibitem{dupuis2018sensitivity}
Paul Dupuis, Markos~A Katsoulakis, Yannis Pantazis, and Luc Rey-Bellet.
\newblock Sensitivity analysis for rare events based on r\'enyi divergence.
\newblock {\em arXiv preprint arXiv:1805.06917}, 2018.

\bibitem{dupuis2019formulation}
Paul Dupuis and Yixiang Mao.
\newblock Formulation and properties of a divergence used to compare
  probability measures without absolute continuity.
\newblock {\em arXiv preprint, arXiv:1911.07422}, 2019.

\bibitem{doi:10.1063/1.5021351}
Jinchao Feng, Joshua Lansford, Alexander Mironenko, Davood~Babaei Pourkargar,
  Dionisios~G. Vlachos, and Markos~A. Katsoulakis.
\newblock Non-parametric correlative uncertainty quantification and sensitivity
  analysis: Application to a langmuir bimolecular adsorption model.
\newblock {\em AIP Advances}, 8(3):035021, 2018.

\bibitem{feng2018non}
Jinchao Feng, Joshua Lansford, Alexander Mironenko, Davood~Babaei Pourkargar,
  Dionisios~G Vlachos, and Markos~A Katsoulakis.
\newblock Non-parametric correlative uncertainty quantification and sensitivity
  analysis: Application to a langmuir bimolecular adsorption model.
\newblock {\em AIP Advances}, 8(3):035021, 2018.

\bibitem{Feng2020Science}
Jinchao Feng, Joshua~L. Lansford, Markos~A. Katsoulakis, and Dionisios~G.
  Vlachos.
\newblock Explainable and trustworthy artificial intelligence for correctable
  modeling in chemical sciences.
\newblock {\em Science Advances}, 6(42), 2020.

\bibitem{friedman2000using}
Nir Friedman, Michal Linial, Iftach Nachman, and Dana Pe'er.
\newblock Using bayesian networks to analyze expression data.
\newblock {\em Journal of computational biology}, 7(3-4):601--620, 2000.

\bibitem{fung1995applying}
Robert Fung and Brendan Del~Favero.
\newblock Applying bayesian networks to information retrieval.
\newblock {\em Communications of the ACM}, 38(3):42--ff, 1995.

\bibitem{2016arXiv160402199G}
Rui {Gao} and Anton~J. {Kleywegt}.
\newblock {Distributionally Robust Stochastic Optimization with Wasserstein
  Distance}.
\newblock {\em arXiv e-prints}, page arXiv:1604.02199, Apr 2016.

\bibitem{Cuturi:short:2017}
Aude {Genevay}, Gabriel {Peyr{\'e}}, and Marco {Cuturi}.
\newblock {GAN and VAE from an Optimal Transport Point of View}.
\newblock {\em arXiv e-prints}, page arXiv:1706.01807, June 2017.

\bibitem{GZ}
Zoubin Ghahramani.
\newblock Probabilistic machine learning and artificial intelligence.
\newblock {\em Nature}, 521(7553):452--459, 2015.

\bibitem{KALE:Gretton:2021}
Pierre {Glaser}, Michael {Arbel}, and Arthur {Gretton}.
\newblock {KALE Flow: A Relaxed KL Gradient Flow for Probabilities with
  Disjoint Support}.
\newblock {\em arXiv e-prints}, page arXiv:2106.08929, June 2021.

\bibitem{doi:10.1287/opre.1090.0795}
Joel Goh and Melvyn Sim.
\newblock Distributionally robust optimization and its tractable
  approximations.
\newblock {\em Operations Research}, 58(4-part-1):902--917, 2010.

\bibitem{gomez2007sensitivity}
Miguel~A G{\'o}mez-Villegas, Paloma Ma{\'\i}n, and Rosario Susi.
\newblock Sensitivity analysis in gaussian bayesian networks using a divergence
  measure.
\newblock {\em Communications in Statistics---Theory and Methods},
  36(3):523--539, 2007.

\bibitem{gomez2013effect}
Miguel~A G{\'o}mez-Villegas, Paloma Main, and Rosario Susi.
\newblock The effect of block parameter perturbations in gaussian bayesian
  networks: Sensitivity and robustness.
\newblock {\em Information Sciences}, 222:439--458, 2013.

\bibitem{gomez2011evaluating}
Miguel~{\'A}ngel G{\'o}mez-Villegas, Paloma Main, Hilario Navarro, and Rosario
  Susi.
\newblock Evaluating the difference between graph structures in gaussian
  bayesian networks.
\newblock {\em Expert Systems with Applications}, 38(10):12409--12414, 2011.

\bibitem{gourgoulias2017biased}
Konstantinos Gourgoulias, M.~Katsoulakis, L.~Rey-Bellet, and J.~Wang.
\newblock How biased is your model? concentration inequalities, information and
  model bias.
\newblock {\em IEEE Transactions on Information Theory}, 66:3079--3097, 2020.

\bibitem{Gunning_Aha_2019}
David Gunning and David Aha.
\newblock Darpa’s explainable artificial intelligence (xai) program.
\newblock {\em AI Magazine}, 40(2):44--58, Jun. 2019.

\bibitem{Hall:Katsoulakis:sparse}
E.~Hall and M.~Katsoulakis.
\newblock Robust information divergences for model-form uncertainty arising
  from sparse data in random pde.
\newblock {\em SIAM/ASA J. Uncertain. Quantification}, 6:1364--1394, 2018.

\bibitem{Hall2021_GINN}
Eric~J. Hall, SÃžren Taverniers, Markos~A. Katsoulakis, and Daniel~M.
  Tartakovsky.
\newblock Ginns: Graph-informed neural networks for multiscale physics.
\newblock {\em Journal of Computational Physics}, 433:110192, 2021.

\bibitem{bookHansenSargent}
Lars~Peter Hansen and Thomas~J. Sargent.
\newblock {\em Robustness}.
\newblock Princeton University Press, stu - student edition edition, 2008.

\bibitem{heckerman2016toward}
David Heckerman, Eric Horvitz, and Bharat~N Nathwani.
\newblock Toward normative expert systems part i.
\newblock {\em Methods of information in medicine}, 31, 2016.

\bibitem{holewinski2012}
Adam Holewinski and Suljo Linic.
\newblock Elementary mechanisms in electrocatalysis: revisiting the orr tafel
  slope.
\newblock {\em Journal of The Electrochemical Society}, 159(11):H864, 2012.

\bibitem{Jiang2016}
Ruiwei Jiang and Yongpei Guan.
\newblock Data-driven chance constrained stochastic program.
\newblock {\em Mathematical Programming}, 158(1):291--327, Jul 2016.

\bibitem{10.5555/2969239.2969284}
Kirthevasan Kandasamy, Akshay Krishnamurthy, Barnab\"{y}s P\'{o}czos, Larry
  Wasserman, and James~M. Robins.
\newblock Nonparametric von mises estimators for entropies, divergences and
  mutual informations.
\newblock In {\em Proceedings of the 28th International Conference on Neural
  Information Processing Systems - Volume 1}, NIPS'15, page 397–405,
  Cambridge, MA, USA, 2015. MIT Press.

\bibitem{Willcox2021}
Michael~G. {Kapteyn}, Jacob V.~R. {Pretorius}, and Karen~E. {Willcox}.
\newblock {A Probabilistic Graphical Model Foundation for Enabling Predictive
  Digital Twins at Scale}.
\newblock {\em arXiv e-prints}, page arXiv:2012.05841, December 2020.

\bibitem{katsoulakis2017scalable}
Markos~A Katsoulakis, Luc Rey-Bellet, and Jie Wang.
\newblock Scalable information inequalities for uncertainty quantification.
\newblock {\em Journal of Computational Physics}, 336:513--545, 2017.

\bibitem{koller2009probabilistic}
Daphne Koller and Nir Friedman.
\newblock {\em Probabilistic graphical models: principles and techniques}.
\newblock MIT press, 2009.

\bibitem{2016arXiv160509349L}
Henry {Lam}.
\newblock {Recovering Best Statistical Guarantees via the Empirical
  Divergence-based Distributionally Robust Optimization}.
\newblock {\em arXiv e-prints}, page arXiv:1605.09349, May 2016.

\bibitem{lazkano2007use}
Elena Lazkano, Basilio Sierra, Aitzol Astigarraga, and Jos{\'e}~Maria
  Martinez-Otzeta.
\newblock On the use of bayesian networks to develop behaviours for mobile
  robots.
\newblock {\em Robotics and Autonomous Systems}, 55(3):253--265, 2007.

\bibitem{levitt1990model}
Tod~S Levitt, John~Mark Agosta, and Thomas~O Binford.
\newblock Model-based influence diagrams for machine vision.
\newblock In {\em Machine Intelligence and Pattern Recognition}, volume~10,
  pages 371--388. Elsevier, 1990.

\bibitem{MILLER20191}
Tim Miller.
\newblock Explanation in artificial intelligence: Insights from the social
  sciences.
\newblock {\em Artificial Intelligence}, 267:1--38, 2019.

\bibitem{MohajerinEsfahani2018}
Peyman Mohajerin~Esfahani and Daniel Kuhn.
\newblock Data-driven distributionally robust optimization using the
  {W}asserstein metric: performance guarantees and tractable reformulations.
\newblock {\em Mathematical Programming}, 171(1):115--166, Sep 2018.

\bibitem{8007086}
Kevin~R. Moon, Kumar Sricharan, and Alfred~O. Hero.
\newblock Ensemble estimation of mutual information.
\newblock In {\em 2017 IEEE International Symposium on Information Theory
  (ISIT)}, pages 3030--3034, 2017.

\bibitem{Muller1997}
Alfred M\"{u}ller.
\newblock Integral probability metrics and their generating classes of
  functions.
\newblock {\em Advances in Applied Probability}, 29(2):429--443, 1997.

\bibitem{Nguyen_Full_2010}
X.~{Nguyen}, M.~J. {Wainwright}, and M.~I. {Jordan}.
\newblock Estimating divergence functionals and the likelihood ratio by convex
  risk minimization.
\newblock {\em IEEE Transactions on Information Theory}, 56(11):5847--5861,
  2010.

\bibitem{Owhadhi:2013}
H.~Owhadi, C.~Scovel, T.~Sullivan, M.~McKerns, and M.~Ortiz.
\newblock Optimal uncertainty quantification.
\newblock {\em SIAM Review}, 55(2):271--345, 2013.

\bibitem{pearl1988probabilistic}
Judea Pearl.
\newblock {\em Probabilistic reasoning in intelligent systems: Networks of
  plausible reasoning}.
\newblock Morgan Kaufmann Publishers, Los Altos, 1988.

\bibitem{pearl2014probabilistic}
Judea Pearl.
\newblock {\em Probabilistic reasoning in intelligent systems: networks of
  plausible inference}.
\newblock Elsevier, 2014.

\bibitem{NIPS2008_ccb09896}
Fernando P\'{e}rez-Cruz.
\newblock Estimation of information theoretic measures for continuous random
  variables.
\newblock In D.~Koller, D.~Schuurmans, Y.~Bengio, and L.~Bottou, editors, {\em
  Advances in Neural Information Processing Systems}, volume~21. Curran
  Associates, Inc., 2009.

\bibitem{Sen:IEEE}
Adil Rasheed, Omer San, and Trond Kvamsdal.
\newblock Digital twin: Values, challenges and enablers from a modeling
  perspective.
\newblock {\em IEEE Access}, 8:21980--22012, 2020.

\bibitem{catalysisGadi}
Gadi Rothenberg.
\newblock {\em Catalysis}.
\newblock John Wiley \& Sons, 2008.

\bibitem{setzler2016activity}
Brian~P Setzler, Zhongbin Zhuang, Jarrid~A Wittkopf, and Yushan Yan.
\newblock Activity targets for nanostructured platinum-group-metal-free
  catalysts in hydroxide exchange membrane fuel cells.
\newblock {\em NATURE NANOTECHNOLOGY}, 11(12):1020, 2016.

\bibitem{10.2307/2632102}
Ross~D. Shachter and C.~Robert Kenley.
\newblock Gaussian influence diagrams.
\newblock {\em Management Science}, 35(5):527--550, 1989.

\bibitem{Smith}
Ralph~C. Smith.
\newblock {\em Uncertainty Quantification: Theory, Implementation, and
  Applications}.
\newblock Society for Industrial and Applied Mathematics, Philadelphia, PA,
  USA, 2013.

\bibitem{spirtes2000causation}
Peter Spirtes, Clark~N Glymour, Richard Scheines, David Heckerman, Christopher
  Meek, Gregory Cooper, and Thomas Richardson.
\newblock {\em Causation, prediction, and search}.
\newblock MIT press, 2000.

\bibitem{suen2017}
Nian-Tzu Suen, Sung-Fu Hung, Quan Quan, Nan Zhang, Yi-Jun Xu, and Hao~Ming
  Chen.
\newblock Electrocatalysis for the oxygen evolution reaction: recent
  development and future perspectives.
\newblock {\em Chemical Society Reviews}, 46(2):337--365, 2017.

\bibitem{natchem}
Jonathan~E. Sutton, Wei Guo, Markos~A. Katsoulakis, and Dionisios~G. Vlachos.
\newblock Effects of correlated parameters and uncertainty in
  electronic-structure-based chemical kinetic modelling.
\newblock {\em NATURE CHEMISTRY}, {8}({4}):331--337, April {2016}.

\bibitem{Katsoulakis_BayesianNetwork}
Kimoon Um, Eric~J. Hall, Markos~A. Katsoulakis, and Daniel~M. Tartakovsky.
\newblock Causality and bayesian network pdes for multiscale representations of
  porous media.
\newblock {\em Journal of Computational Physics}, 394:658--678, 2019.

\bibitem{4035959}
Qing Wang, Sanjeev~R. Kulkarni, and Sergio Verdu.
\newblock A nearest-neighbor approach to estimating divergence between
  continuous random vectors.
\newblock In {\em 2006 IEEE International Symposium on Information Theory},
  pages 242--246, 2006.

\bibitem{4839047}
Qing Wang, Sanjeev~R. Kulkarni, and Sergio Verdu.
\newblock Divergence estimation for multidimensional densities via
  $k$-nearest-neighbor distances.
\newblock {\em IEEE Transactions on Information Theory}, 55(5):2392--2405,
  2009.

\bibitem{w06}
Larry Wasserman.
\newblock {\em All of Nonparametric Statistics}.
\newblock Springer, New York, NY, 2006.

\bibitem{wasserman2013all}
Larry Wasserman.
\newblock {\em All of statistics: a concise course in statistical inference}.
\newblock Springer Science \& Business Media, 2013.

\bibitem{doi:10.1287/opre.2014.1314}
Wolfram Wiesemann, Daniel Kuhn, and Melvyn Sim.
\newblock Distributionally robust convex optimization.
\newblock {\em Operations Research}, 62(6):1358--1376, 2014.

\bibitem{doi:10.1137/16M1094725}
W.~Xie and S.~Ahmed.
\newblock On deterministic reformulations of distributionally robust joint
  chance constrained optimization problems.
\newblock {\em SIAM Journal on Optimization}, 28(2):1151--1182, 2018.

\end{thebibliography}

